Performance Evaluation of Container-based Virtualization for High Performance Computing Environments

Virtualization technologies have evolved along with the development of computational environments since virtualization offered needed features at that time such as isolation, accountability, resource allocation, resource fair sharing and so on. Novel processor technologies bring to commodity computers the possibility to emulate diverse environments where a wide range of computational scenarios can be run. Along with processors evolution, system developers have created different virtualization mechanisms where each new development enhanced the performance of previous virtualized environments. Recently, operating system-based virtualization technologies captured the attention of communities abroad (from industry to academy and research) because their important improvements on performance area. In this paper, the features of three container-based operating systems virtualization tools (LXC, Docker and Singularity) are presented. LXC, Docker, Singularity and bare metal are put under test through a customized single node HPL-Benchmark and a MPI-based application for the multi node testbed. Also the disk I/O performance, Memory (RAM) performance, Network bandwidth and GPU performance are tested for the COS technologies vs bare metal. Preliminary results and conclusions around them are presented and discussed.

==> Ideas.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%	Just a bunch of random ideas	%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Not all user namespaces are equal, and Singularity does swap out the user namespaces so if the container have more efficient libraries than on the host that could yield a performance increase. 

Another one is on metadata IO lookups. 


if you have a program that does lots of iops. 
Container images can be much more optimal then running against shared storage. (even when the container image exists on that remote storage)
% see : https://github.com/wresch/python_import_problem/
%
%%Network
%
To avoid users of having root access, Docker must be isolated thus will preclude access to high performance networks (e.g. InfiniBand) and optimized storage platforms.

%
%% Slack chat ideas
%
make our point on the fact that containers can play the HPC game.  rather than some say that containers have some work to do before going HPC.

talk about some performance gains that can be taken from the use of containers. as the metadata lookup, and the optimized libraries inside a non-optimized host

results can be significantly different depending on the architecture Particularly for the HPL tests where we get important differences

GPU tests. so we can talk about the next cloud computing gen that is comming with GPU, and how containers can be used in that scenario

==> Tentative_Journals.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%	Tentative Journals to submit the paper %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% see http://www.guide2research.com/journals/list-2016.pdf

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Performance Evaluation functions as a leading journal in the area of modeling, measurement, and evaluation of performance aspects of computing and communication systems. As such, it aims to present a balanced and complete view of the entire Performance Evaluation profession.

https://www.journals.elsevier.com/performance-evaluation/
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The Journal of Information Technology (JIT) is a top-ranked journal in its field, focused on new research addressing technology and the management of IT - including strategy, change, infrastructure, human resources, sourcing, system development and implementation, communications, technology developments, technology futures, national policies and standards, as well as articles that advance understanding and application of research approaches and methods.

http://www.springer.com/business+%26+management/journal/41265
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Information Sciences will publish original, innovative and creative research results. A smaller number of timely tutorial and surveying contributions will be published from time to time.

https://www.journals.elsevier.com/information-sciences/
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PeerJ Computer Science is the new open access journal covering all subject areas in computer science, with the backing of a prestigious advisory board and more than 300 academic editors.

https://peerj.com/computer-science/
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MIS Quarterly: Management Information Systems

The editorial objective of the MIS Quarterly is the enhancement and communication of knowledge concerning the development of IT-based services, the management of IT resources, and the use, impact, and economics of IT with managerial, organizational, and societal implications. Professional issues affecting the IS field as a whole are also in the purview of the journal.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Future Generation Computer Systems

Computing infrastructures and systems are rapidly developing and so are novel ways to map, control and execute scientific applications which become more and more complex and collaborative.
Computational and storage capabilities, databases, sensors, and people need true collaborative tools. Over the last years there has been a real explosion of new theory and technological progress supporting a better understanding of these wide-area, fully distributed sensing and computing systems. Big Data in all its guises require novel methods and infrastructures to register, analyze and distill meaning.

FGCS aims to lead the way in advances in distributed systems, collaborative environments, high performance and high performance computing, Big Data on such infrastructures as grids, clouds and the Internet of Things (IoT). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

PLOS ONE or PLOS COMPUTIONAL BIOLOGY ? But that second journal would need to refactor a lot and focus on biology applications... And PLOS ONE is a big journal...

==> results.tex <==
\section{Results}
